Augmenting Monte Carlo Dropout Classification Models with Unsupervised Learning Tasks for Detecting and Diagnosing Out-of-Distribution Faults

The Monte Carlo dropout method has proved to be a scalable and easy-to-use approach for estimating the uncertainty of deep neural network predictions. This approach was recently applied to Fault Detection and Di-agnosis (FDD) applications to improve the classification performance on incipient faults. In this paper, we propose a novel approach of augmenting the classification model with an additional unsupervised learning task. We justify our choice of algorithm design via an information-theoretical analysis. Our experimental results on three datasets from diverse application domains show that the proposed method leads to improved fault detection and diagnosis performance, especially on out-of-distribution examples including both incipient and unknown faults.

==> macros.tex <==
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography

% \usepackage{cite}
\usepackage{acronym}
\usepackage{amsmath,amssymb,amsfonts,bm}
% \usepackage{dsfont}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{gensymb}
\usepackage[font=footnotesize]{subcaption}
% \usepackage{todonotes}

\usepackage{etoolbox}
\usepackage{comment}

\newtoggle{anonymous}
\settoggle{anonymous}{true} %set true to show all comments, set false to hide all comments

\newtoggle{comments}
\settoggle{comments}{false} %set true to show all comments, set false to hide all comments
% Comment region command (from Wesley Willett)
\iftoggle{comments}{
  %if we want to show comments
  %% ============================================================
  %% add your names here
  %% possible colors include:
  %%   Orange, magenta, NavyBlue, violet, BrickRed, OliveGreen
  %% ============================================================
  \newcommand {\alberto}[1]{{\color{orange}{~Alberto: #1}\normalfont}}
  \newcommand {\bjin}[1]{{\color{blue}{~Baihong: #1}\normalfont}}
  \newcommand {\yuxin}[1]{{\color{violet}{~Yuxin: #1}\normalfont}}
  \newcommand {\yingshui}[1]{{\color{green}{~Yingshui: #1}\normalfont}}
  \newcommand {\alex}[1]{{\color{cyan}{~Alex: #1}\normalfont}}
  \newcommand {\red}[1]{{\color{red}{#1}\normalfont}}
}{
  \newcommand {\alberto}[1]{{}}
  \newcommand {\bjin}[1]{{}}
  \newcommand {\yuxin}[1]{{}}
  \newcommand {\alex}[1]{{}}
  \newcommand {\yingshui}[1]{{}}
  \newcommand {\red}[1]{{}}
}

\newcommand{\Score}{f_\text{score}}
\newcommand{\expctover}[2]{\mathbb{E}_{#1}\!\left[#2\right]}
\newcommand{\unit}[1]{\mathds{1}\left\{#1\right\}}


\acrodef{SVM}{Support Vector Machine}
\acrodef{AE}{AutoEncoder}
\acrodef{RNN}{Recurrent Neural Network}
\acrodef{CNN}{Convolutional Neural Network}
\acrodef{OC-SVM}{One-class Support Vector Machine}
\acrodef{CPS}{Cyber-Physical System}
\acrodef{FDD}{Fault Detection and Diagnosis}
\acrodef{LDA}{Linear Discriminant Analysis}
\acrodef{PCA}{Principal Component Analysis}
\acrodef{MSE}{Mean Square Error}
\acrodef{LAMPS}{Laser Additive Manufacturing Pilot System}
\acrodef{AM}{Additive Manufacturing}
\acrodef{SLS}{Selective Laser Sintering}
\acrodef{IR}{infrared}
\acrodef{IoT}{Internet of Things}
\acrodef{ROC}{Receiver Operating Characteristic}
\acrodef{RMS}{Root-Mean-Square}
\acrodef{AUC}{Area Under the Curve}
